On the Hyperbolicity of Lorenz Renormalization

We consider infinitely renormalizable Lorenz maps with real critical exponent $\alpha>1$ and combinatorial type which is monotone and satisfies a long return condition. For these combinatorial types we prove the existence of periodic points of the renormalization operator, and that each map in the limit set of renormalization has an associated unstable manifold. An unstable manifold defines a family of Lorenz maps and we prove that each infinitely renormalizable combinatorial type (satisfying the above conditions) has a unique representative within such a family. We also prove that each infinitely renormalizable map has no wandering intervals and that the closure of the forward orbits of its critical values is a Cantor attractor of measure zero.

==> inv-meas.tex <==
\section{Invariant measures} % (fold)
\label{sec:inv-meas}

Let $f$ be an infinitely renormalizable map of any combinatorial
type\footnote{Contrary to other sections, in this section we consider general
combinatorial types and not just monotone types.} and let $\Lambda$ be the
closure of the orbits of the critical values and assume that this is a Cantor
set (in \secref{apb} we prove that $\Lambda$ is a Cantor set, although our
proof is only valid for some combinatorial types).  In this section we describe
the invariant measures supported on~$\Lambda$.  The techniques employed are an
adaptation of~\citep{GM06} which also contains proofs for all the statements we
choose not to provide proofs for here.

\begin{theorem} \label{thm:inv-meas}
  If $f$ is infinitely renormalizable (of any combinatorial type) with a Cantor
  attractor~$\Lambda$, then $\Lambda$ supports one or two ergodic invariant
  probability measures. \index{invariant measure}
  
  If the combinatorial type of~$f$ is bounded then $\Lambda$ is \Index{uniquely
  ergodic}.  Furthermore, it is possible to choose the combinatorial type so
  that $\Lambda$ has two distinct ergodic invariant probability measures.
\end{theorem}

\begin{remark}
  Bounded combinatorial type is sufficient for $\Lambda$ to be uniquely
  ergodic, but is not necessary as \exref{inv-meas} shows.
\end{remark}

An infinitely renormalizable map naturally defines a sequence of finer and
finer covers of~$\Lambda$.  We now describe the construction of these covers
and how they in turn can be identified with certain directed graphs.

\begin{definition}
  Since $f$ is infinitely renormalizable we get a nested sequence
  of nice intervals $\{C_n\}$.  Let $a_n =\tau(\lcv)$ and $b_n = \tau(\rcv)$
  denote the transfer times of the critical values to the nice
  interval~$C_n$.  Let $\{U_n^i\}$ and $\{V_n^i\}$ be the pull-backs of $C_n$
  along the orbits of the critical values, that is
  \begin{gather*}
    f^{i-1}(\lcv) \in U_n^i \quad\text{and}\quad f^{a_n+1-i}(U_n^i) = C_n,
    \quad i=1,\dots,a_n+1, \\
    f^{i-1}(\rcv) \in V_n^i \quad\text{and}\quad f^{b_n+1-i}(V_n^i) = C_n,
    \quad i=1,\dots,b_n+1.
  \end{gather*}
\end{definition}

The intervals $\{U_n^i\}$ and $\{V_n^j\}$ cover the Cantor set~$\Lambda$ and
they satisfy a disjointness property expressed by the following lemma.
Intuitively, for a fixed~$n$ these sets are pairwise disjoint except that if
they overlap at some time, then all remaining intervals follow the same orbit.

\begin{lemma}
  There exists $k_n \geq 0$ such that $U_n^{a_n+1-i} = V_n^{b_n+1-i}$ for $i =
  0,\dots,k_n$, and
  \[
    \Lambda'_n = \{U_n^i\}_{i=1}^{a_n-k_n} \cup \{V_n^i\}_{i=1}^{b_n+1}
  \]
  is a pairwise disjoint cover of $\Lambda$ for all~$n$.
\end{lemma}

\begin{remark}
  Note that $k_n = 0$ if $f$ has monotone combinatorial type.
\end{remark}

\begin{proof}
  Since $C_n$ is nice it follows that if $U_n^{a_n+1-k} \cap V_n^{b_n+1-k} \neq
  \emptyset$ for some $k$, then $U_n^{a_n+1-i} = V_n^{b_n+1-i}$ for all $i =
  0,\dots,k$.  Define $k_n$ to be the largest such~$k$ (which exists since
  $U_n^{a_n+1} = C_n = V_n^{b_n+1}$).

  By \propref{Tbranches} $\{U_n^i\}_i$ is a pairwise disjoint collection and so
  is $\{V_n^i\}_i$ which proves the disjointness property of~$\Lambda'_n$.

  Finally, $\Lambda'_n$ covers $\Lambda$ since the critical values are
  contained in $U_n^1$ and $V_n^1$, both of which are eventually mapped
  inside~$C_n$.
\end{proof}

\begin{definition}
  The $n$--th cover of~$\Lambda$ is defined by
  \[
    \Lambda_n = \{ I \cap \Lambda \mid I \in \Lambda'_n \}.
  \]
  The covers come with natural projections
  \[
    \pi_{ij}: \Lambda_j \to \Lambda_i, \quad i \leq j,
  \]
  defined by $I = \pi_{ij}(J)$, where $I \in \Lambda_i$ is the unique element
  which contains $J \in \Lambda_j$.  These projections satisfy
  $\pi_{ii} = \id$ and $\pi_{ij} = \pi_{ik} \circ \pi_{kj}$ if $i
  \leq k \leq j$.  Hence we get an inverse system
  $(\{\Lambda_i\}_i,\{\pi_{ij}\}_{i \leq j})$.  The inverse limit of this system
  can be identified with $\Lambda$ via the natural projections
  \[
    p_n: \Lambda \to \Lambda_n,
  \]
  defined by $p_n(x) = I$, where $I \in \Lambda_n$ is the unique element
  containing~$x \in \Lambda$.
  Explicitly, $p: \Lambda \to \varprojlim \Lambda_n$ is defined by
  \[
    p(x) = (p_1(x),p_2(x),\dots).
  \]
\end{definition}

\begin{remark}
  Note that $p$ is:
  \begin{inparaenum}[(i)]
    \item well-defined, since $p_i = \pi_{ij} \circ p_j$,
    \item surjective, since if $(x_i)_i \in \varprojlim \Lambda_n$ then
      $x = \lim x_i$ exists and $p(x) = (x_1,x_2,\dots)$,
    \item injective, since if $x,y \in \Lambda$ are distinct then $p_n(x) \neq
      p_n(y)$ for some $n$ due to the fact that the diameter of elements in
      $\Lambda_n$ tends to zero as $n \to \infty$.
  \end{inparaenum}
\end{remark}

We think of $\Lambda_n$ as the directed graph where each element in $\Lambda_n$
is a node and where an edge connects $I$ to~$J$ if and only if $f(I) \cap J
\neq \emptyset$.  Note that if there is an edge from $I$ to $J$, then $f(I) =
J$ unless $I = \zero_n =  C_n \cap \Lambda$.  The image of $\zero_n$ is
contained in the nodes $\one_n^1 = U_n^1 \cap \Lambda$ and $\one_n^2 = V_n^1
\cap \Lambda$.  For example, $\Lambda_n$ could look like:

\begin{center}
  \begin{tikzpicture}
    [node distance=0.5cm,
     special/.style={
        text height=1.5ex,text depth=.25ex,
        rectangle,draw,rounded corners=1mm}]
        %top color=white, bottom color=black!10}]
    \node (Z)  [special] {$\zero_n = C_n \cap \Lambda$};
    \node (E1) [special,above right=of Z] {$\one_n^1 = U_n^1\cap\Lambda$}
      edge [<-,bend left=20] (Z.east);
    \node (E2) [special,below right=of Z] {$\one_n^2 = V_n^1\cap\Lambda$}
      edge [<-,bend right=20] (Z.east);
    \node (u1) [special,left=of E1] {$U_n^2\cap\Lambda$}
      edge [<-] (E1);
    \node (u2) [special,left=of Z] {$U_n^3\cap\Lambda = V_n^5\cap\Lambda$}
      edge [<-,bend left=15] (u1)
      edge [->] (Z);
    \node (v1) [special,left=of E2] {$V_n^2\cap\Lambda$}
      edge [<-] (E2);
    \node (v2) [special,left=of v1] {$V_n^3\cap\Lambda$}
      edge [<-] (v1);
    \node (v3) [special,left=of v2] {$V_n^4\cap\Lambda$}
      edge [<-] (v2)
      edge [->] (u2);
  \end{tikzpicture}
  %\begin{tikzpicture}
  %  \tikzstyle{every node}=[draw,shape=circle];
  %  \node (Z) at (0,0) [inner sep=0.5mm] {$\zero_n$};
  %  \node (E1) at (30:1.2) [inner sep=0.5mm] {$\one_n^1$}
  %    edge [<-] (Z);
  %  \node (E2) at (-30:1.2) [inner sep=0.5mm] {$\one_n^2$}
  %    edge [<-] (Z);
  %  \node (u1) at (105:1.2) {}
  %    edge [<-,bend left=30] (E1);
  %  \node (u2) at (180:1.2) {}
  %    edge [<-,bend left=30] (u1)
  %    edge [->] (Z);
  %  \node (v1) at (-67.5:1.2) {}
  %    edge [<-,bend right=10] (E2);
  %  \node (v2) at (-105:1.2) {}
  %    edge [<-,bend right=10] (v1);
  %  \node (v3) at (-142.5:1.2) {}
  %    edge [<-,bend right=20] (v2)
  %    edge [->,bend left=20] (u2);
  %\end{tikzpicture}
\end{center}

We now describe how the invariant measures on $\Lambda$ can be identified with
a subset of an inverse limit of ``almost invariant'' measures on~$\Lambda_n$.
We define the ``almost invariant'' signed measures on $\Lambda_n$ as follows.

\begin{definition}
  Let $\Sigma_n$ be the $\sigma$--algebra generated by $\Lambda_n$.  Note that
  $\Lambda_n$ consists of exactly two loops, by which we mean a maximal
  collection $\{I_k \in \Lambda_n\}_k$ such that $f(I_k) = I_{k+1}$ or $I_k =
  \zero_n$.  These loops start in $\one_n^i$ and terminate in $\zero_n$.  Each
  loop defines a \Index{loop measure},
  \[
    \nu_n^i: \Sigma_n \to \reals,
  \]
  by $\nu_n^i(I) = 1$ if and only if $I$ is a node on the $i$--th loop
  of~$\Lambda_n$.

  Let $H_1(\Lambda_n)$ denote $\reals$--module generated by
  $\{\nu_n^1,\nu_n^2\}$
  and let $\meas(\Lambda)$ denote the $\reals$--module of signed invariant
  measures on~$\Lambda$.
\end{definition}

\begin{remark}
  Note that the (signed) measures in $H_1(\Lambda_n)$ are almost invariant
  since $\nu_n^i(f\inv(I)) = \nu_n^i(I)$ if $I \in \Lambda_n \setminus
  \{\one_n^1,\one_n^2\}$, but invariance fails since $f^{-1}(\one_n^i) \notin
  \Sigma_n$.  The notation $H_1(\Lambda_n)$ comes from the fact that
  $H_1(\Lambda_n)$ is isomorphic to the first homology module of the
  graph~$\Lambda_n$.
\end{remark}

Now consider the \Index{push-forward}
\[
  (p_n)_*\mu = \mu \circ p_n\inv
\]
of $\mu \in \meas(\Lambda)$ under the projection $p_n$:

\begin{lemma}
  The push-forward of $p_n$ is a homomorphism $(p_n)_*: \meas(\Lambda) \to
  H_1(\Lambda_n)$ and
  \[
    (p_n)_*(\mu) = \mu(\one_n^1) \nu_n^1 + \mu(\one_n^2) \nu_n^2.
  \]
\end{lemma}

The push-forward under the projections $\pi_{ij}$ induces an inverse system
\[
  (\{H_1(\Lambda_i)\}_i,\{(\pi_{ij})_*\}_{i \leq j}).
\]
Because of the
previous lemma and the identification of $\Lambda$ with $\varprojlim
\Lambda_n$, the inverse limit $\varprojlim H_1(\Lambda_n)$ is isomorphic to
$\meas(\Lambda)$ via the isomorphism
\[
  p_*(\mu) = \big((p_1)_*\mu,(p_2)_*\mu,\dots\big).
\]

\begin{definition}
  Let $\invmeas(\Lambda) \subset \meas(\Lambda)$ denote the subset of positive
  invariant measures.
\end{definition}

Using the above one can check that $\invmeas(\Lambda)$ is identified with
$\varprojlim H_1^+(\Lambda_n)$, where
\[
  H_1^+(\Lambda_n) = \big\{ x_1 \nu_n^1 + x_2 \nu_n^2 \mid x_i \geq 0 \big\}
\]
are the (positive) almost invariant measures on~$\Lambda_n$.

\begin{lemma}
  Let $W_n = (w_{ij})$ be the winding matrix defined by
  \[
    w_{ij} = \#\{I \subset E_n^i \mid I\text{ is an element of the $j$--th loop
      of }\Lambda_n\}.
  \]
  Then $W_n$ is the representation of the push-forward $(\pi_{n,n+1})_*$ if we
  use the loop measures $\{\nu_k^1,\nu_k^2\}$ as bases of $H_1(\Lambda_k)$, for
  $k=n,n+1$.
\end{lemma}

\begin{proof}[Proof of~\thmref{inv-meas}]
  By the above every invariant measure is represented by an
  inverse limit
  \[
    \{(z_1,z_2,\dots) \mid z_i = W_i z_{i+1}, z_i \in K \},
  \]
  where $K \subset \reals^2$ is the cone $\{(x_1,x_2) \mid x_i\geq0\}$.  This
  suggests that we should look at the sets
  \[
    I_n = \bigcap_{m>n} W_n \dotsm W_{m-1} K,
  \]
  since $z_n \in I_n$.  The winding matrices have positive integer entries, so
  either $I_n$ is a one-dimensional or a two-dimensional subspace, for all
  $n\geq1$.

  If $I_n$ has dimension two then it is the convex hull of two points and hence
  $I_n \cap \{x_1+x_2=1\}$ has exactly two extremal points.  This implies that
  there are two ergodic invariant probability measures.  Since $I_n$ cannot
  have have dimension higher than two, this also shows that there can be no
  more than two ergodic invariant probability measures.  In \exref{inv-meas} we
  construct a map with exactly two ergodic invariant probability
  measures.

  To see that $\Lambda$ is uniquely ergodic in the bounded combinatorial type
  case we introduce the \Index{Hilbert metric} (also known as the
  \Index{hyperbolic metric}) on the interior of~$K$.  This metric is defined as
  in the following figure:
  %\[
  %  \distance(z,z') = \log \left\{
  %  1 + \frac{\abs{z-z'}\abs{w-w'}}{\abs{w-z}\abs{z'-w'}} \right\},
  %  \qquad z,z' \in \intr K,
  %\]
  \begin{center}
    \begin{tikzpicture}[scale=1]
      \path coordinate (beg) at (-0.5,2.25)
            coordinate (w) at (0,2)
            coordinate (z) at (1,1.5)
            coordinate (zp) at (3,0.5)
            coordinate (wp) at (4,0)
            coordinate (end) at (4.5,-0.25);

      \draw [->] (-0.5,0) -- (5,0) node [below] {$x_1$};
      \draw [->] (0,-0.5) -- (0,3) node [left] {$x_2$};

      \draw (beg) -- (w) -- (z) -- (zp) -- (wp) -- (end);
      \filldraw (w) circle (1.5pt) node [above right] {$w$};
      \filldraw (z) circle (1.5pt) node [above right] {$z$};
      \filldraw (zp) circle (1.5pt) node [above right] {$z'$};
      \filldraw (wp) circle (1.5pt) node [above right] {$w'$};

      \draw (4,1.5) node [above right] {%
        $\distance(z,z') = \log \left\{%
        1 + \frac{\abs{z-z'}\abs{w-w'}}{\abs{w-z}\abs{z'-w'}} \right\}$%
      };
    \end{tikzpicture}
  \end{center}
  Here $w$ and $w'$ are the points on~$\bndry K$ closest to $z$ and $z'$,
  respectively, on the line through $z$ and~$z'$.  Note that $\distance(z,z')$
  equals the log of one plus the cross-ratio of $(w,z,z',w')$.  The cross-ratio
  is well-defined since these four points are collinear.  The Hilbert metric is
  contracted by positive matrices because:
  \begin{inparaenum}[(i)]
    \item linear maps preserve cross-ratio,
    \item $W K \subset K$, if $W$ is a positive matrix, and
    \item the cross-ratio of $(w,z,z',w')$ decreases if $w$ is moved further
      away from $z$ on the line through these four points (and similarly for
      $w'$ and~$z'$).
  \end{inparaenum}

  If $f$ has bounded combinatorial type, then there is a bound on the
  contraction constant for the winding matrices~$W_n$ which is independent
  of~$n$.  This implies that $I_n$ is one-dimensional and hence there is a
  unique ergodic probability measure.
\end{proof}

\begin{example} \label{ex:inv-meas}
  If $f$ is of \emph{monotone} combinatorial type
  $\{(\omega_n^-,\omega_n^+)\}_{n\geq0}$ with $a_n = \abs{\omega_n^-}-1$ and
  $b_n = \abs{\omega_n^+}-1$, then we can compute the winding matrix:
  \[
    W_n = \begin{pmatrix}
      1       & b_{n+1} \\
      a_{n+1} & 1
    \end{pmatrix}.
  \]
  Thus
  \begin{align*}
    W_{n-1} W_n &= \begin{pmatrix}
      1 + a_{n+1} b_n & b_n + b_{n+1} \\
      a_n + a_{n+1} & 1 + a_n b_{n+1}
    \end{pmatrix} \\
    &= a_n b_n \begin{pmatrix}
      s_n + (a_nb_n)\inv & a_n\inv (1+r_n) \\
      b_n\inv(1+s_n) & r_n + (a_nb_n)\inv
    \end{pmatrix}
  \end{align*}
  where $s_n = a_{n+1}/a_n$ and $r_n = b_{n+1}/b_n$.  Assuming
  $a_n,b_n\to\infty$ we see that the above matrix modulo the multiplicative
  term is asymptotically equal to
  \[
    \begin{pmatrix}
      s_n & 0 \\
      0 & r_n
    \end{pmatrix}.
  \]
  If we let
  \[
    I_n^m =
    \bigcap_{i=n}^m \big(W_n W_{n+1}\big) \dotsm \big(W_m W_{m+1}\big) K,
  \]
  then $I_n^m$ is two-dimensional for all $m$ if we let $a_n$
  and~$b_n$ grow sufficiently fast.  Thus the sets $I_n$ in the proof
  of \thmref{inv-meas} will be two-dimensional, giving rise to two ergodic
  invariant probability measures.

  It is possible to compute the contraction constant of the Hilbert metric in
  this example \citep[see][]{Bus73}.  It is given by
  \[
    k_{n-1} = \frac{\sqrt{a_n b_n} - 1}{\sqrt{a_n b_n} + 1}.
  \]
  This constant is an exact bound on the contraction, meaning that there exist
  $x$, $y$ such that $\distance(W_nx,W_ny) = k_n \distance(x,y)$.

  By choosing $a_n$ and~$b_n$ such that $\prod k_n = 0$ we get that the sets
  $I_n$ are lines which means that $\Lambda$ is uniquely ergodic.
  In particular, we could choose $\{a_n\}$ and~$\{b_n\}$ unbounded but growing
  slowly enough for $\prod k_n = 0$ to hold, hence showing that bounded
  combinatorial type is not necessary for $\Lambda$ to be uniquely ergodic.
\end{example}

% section Invariant measures (end)


==> references.tex <==
\begin{bibdiv}
\begin{biblist}

\bib{B}{article}{
   author={Bushell, P. J.},
   title={Hilbert's metric and positive contraction mappings in a Banach
   space},
   journal={Arch. Rational Mech. Anal.},
   volume={52},
   date={1973},
   pages={330--338},
   issn={0003-9527},
   %review={\MR{0336473 (49 \#1247)}},
}

\bib{GM}{article}{
  author={Gambaudo, Jean-Marc},
  author={Martens, Marco},
  title={Algebraic topology for minimal Cantor sets},
  journal={Ann. Henri Poincar\'e},
  volume={7},
  date={2006},
  number={3},
  pages={423--446},
  issn={1424-0637},
  %review={\MR{2226743 (2006m:37007)}},
  %doi={10.1007/s00023-005-0255-3},
}

\bib{GD}{book}{
   author={Granas, Andrzej},
   author={Dugundji, James},
   title={Fixed point theory},
   series={Springer Monographs in Mathematics},
   publisher={Springer-Verlag},
   place={New York},
   date={2003},
   pages={xvi+690},
   isbn={0-387-00173-5},
   %review={\MR{1987179 (2004d:58012)}},
}

\bib{Jia96}{book}{
   author={Jiang, Yunping},
   title={Renormalization and geometry in one-dimensional and complex
   dynamics},
   series={Advanced Series in Nonlinear Dynamics},
   volume={10},
   publisher={World Scientific Publishing Co. Inc.},
   place={River Edge, NJ},
   date={1996},
   pages={xvi+309},
   isbn={981-02-2326-9},
   %review={\MR{1442953 (98e:58070)}},
}

\bib{KH95}{book}{
   author={Katok, Anatole},
   author={Hasselblatt, Boris},
   title={Introduction to the modern theory of dynamical systems},
   series={Encyclopedia of Mathematics and its Applications},
   volume={54},
   note={With a supplementary chapter by Katok and Leonardo Mendoza},
   publisher={Cambridge University Press},
   place={Cambridge},
   date={1995},
   pages={xviii+802},
   isbn={0-521-34187-6},
   %review={\MR{1326374 (96c:58055)}},
}


\bib{Mar94}{article}{
   author={Martens, Marco},
   title={Distortion results and invariant Cantor sets of unimodal maps},
   journal={Ergodic Theory Dynam. Systems},
   volume={14},
   date={1994},
   number={2},
   pages={331--349},
   issn={0143-3857},
   %review={\MR{1279474 (96c:58108)}},
   %doi={10.1017/S0143385700007902},
}

\bib{Mar98}{article}{
   author={Martens, Marco},
   title={The periodic points of renormalization},
   journal={Ann. of Math. (2)},
   volume={147},
   date={1998},
   number={3},
   pages={543--584},
   issn={0003-486X},
   %review={\MR{1637651 (99h:58057)}},
   %doi={10.2307/120959},
}

\bib{MM}{article}{
   author={Martens, Marco},
   author={de Melo, Welington},
   title={Universal models for Lorenz maps},
   journal={Ergodic Theory Dynam. Systems},
   volume={21},
   date={2001},
   number={3},
   pages={833--860},
   issn={0143-3857},
   %review={\MR{1836435 (2002d:37057)}},
   %doi={10.1017/S0143385701001420},
}

\bib{MMS}{article}{
   author={Martens, Marco},
   author={de Melo, Welington},
   author={van Strien, Sebastian},
   title={Julia-Fatou-Sullivan theory for real one-dimensional dynamics},
   journal={Acta Math.},
   volume={168},
   date={1992},
   number={3-4},
   pages={273--318},
   issn={0001-5962},
   %review={\MR{1161268 (93d:58137)}},
   %doi={10.1007/BF02392981},
}

\bib{ODD}{book}{
   author={de Melo, Welington},
   author={van Strien, Sebastian},
   title={One-dimensional dynamics},
   series={Ergebnisse der Mathematik und ihrer Grenzgebiete (3) [Results in
   Mathematics and Related Areas (3)]},
   volume={25},
   publisher={Springer-Verlag},
   place={Berlin},
   date={1993},
   pages={xiv+605},
   isbn={3-540-56412-8},
   %review={\MR{1239171 (95a:58035)}},
}

\bib{Mis}{article}{
   author={Misiurewicz, Micha{\l}},
   title={Absolutely continuous measures for certain maps of an interval},
   journal={Inst. Hautes \'Etudes Sci. Publ. Math.},
   number={53},
   date={1981},
   pages={17--51},
   issn={0073-8301},
   %review={\MR{623533 (83j:58072)}},
}

\bib{PT93}{book}{
   author={Palis, Jacob},
   author={Takens, Floris},
   title={Hyperbolicity and sensitive chaotic dynamics at homoclinic
   bifurcations},
   series={Cambridge Studies in Advanced Mathematics},
   volume={35},
   note={Fractal dimensions and infinitely many attractors},
   publisher={Cambridge University Press},
   place={Cambridge},
   date={1993},
   pages={x+234},
   isbn={0-521-39064-8},
   %review={\MR{1237641 (94h:58129)}},
}

\end{biblist}
\end{bibdiv}

